PAGANI: A Parallel Adaptive GPU Algorithm for Numerical

We present a new adaptive parallel algorithm for the challenging problem of multi-dimensional numerical integration on massively parallel architectures. Adaptive algorithms have demonstrated the best performance, but efficient many-core utilization is difficult to achieve because the adaptive work-load can vary greatly across the integration space and is impossible to predict a priori. Existing parallel algorithms utilize sequential computations on independent processors, which results in bottlenecks due to the need for data redistribution and processor synchronization. Our algorithm employs a high-throughput approach in which all existing sub-regions are processed and sub-divided in parallel. Repeated sub-region classification and filtering improves upon a brute-force approach and allows the algorithm to make efficient use of computation and memory resources. A CUDA implementation shows orders of magnitude speedup over the fastest open-source CPU method and extends the achievable accuracy for difficult integrands. Our algorithm typically outperforms other existing deterministic parallel methods.

==> Parallel_Adaptive_MD_Integration (1)/integral_test_suite_table.tex <==
\begin{table*}[t]
\caption{Integral Test Suite}
\centering
\begin{tabular}{|c|l|c|c|}
\hline
{\textbf{ID}} & \multicolumn{1}{c|}{{\textbf{Integrand}}} & {\textbf{d}} & Integral \\ \hline
Box s=15 & $(\sum_{i=1}^{d} {x_i}^2)^{s/2}  $ & 8 & 8.87985117541348e3 \\ \hline
Box s=22 & $ (\sum_{i=1}^{d} {x_i}^2)^\frac{22}{2}  $ & 8 & 1.49536928375722e6 \\ \hline
% \multirow{Corner Peak} & $ (1+ \sum_{i=1}^{d} i\cdot x_i)^{-d-1} $ & 3 & $1.08465608465608e-2$ \\ \cline{2-4}
%  & $ (1+ \sum_{i=1}^{d} i\cdot x_i)^{-d-1}$ & 6 & 7.17901606381999e-7 \\ \cline{2-4}
%  & $ (1+ \sum_{i=1}^{d} i\cdot x_i)^{-9} $ & 8 & 2.27519658179178e-10 \\ \hline
% \multirow{Gaussian} & $ e^{-625 \cdot \sum_{i=1}^{d} (x_i-.5)^2}$ & 5 & 1.79132603674879e-6 \\ \cline{2-4}
%  & $ e^{-625 \cdot \sum_{i=1}^{d} (x_i-.5)^2}$ & 8 & 6.38380219000438e-10 \\ \hline
% \multirow{$C^0$} & $-10  \sum_{i=1}^{d} \lvert x_i - .5 \rvert$ & 2 & 3.94627802372637e-2 \\ \cline{2-4}
%  & $-10  \sum_{i=1}^{d} \lvert x_i - .5 \rvert$ & 5 & 3.093636e-4 \\ \cline{2-4}
%  & $-10  \sum_{i=1}^{d} \lvert x_i - .5 \rvert$ & 8 & 2.42521762564189e-6 \\ \hline
% Discontinuous & \begin{tabular}[c]{@{}l@{}}$\begin{cases}\\ 0, & \text{if} z > .9 \\ 0 & \text{if} y > .8 \\ 0 & \text{if} x > .7 \\ 0 & \text{if} w> ,6 \\ 0 & \text{if} v > .5 \\ 0 & \text{if} u > .4\\ e^{10\cdotz + 9\cdoty + 8\cdotx + 7\cdotw + 6\cdotv + 5\cdotu}, \text{otherwise}\\ \end{cases}\\ $\end{tabular} & 6 & 1.54773678850912e8 \\ \hline
\end{tabular}
\end{table*}

==> Parallel_Adaptive_MD_Integration (1)/summary_results_table.tex <==
\begin{table*}[t]
\centering
\caption{Summary Results}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
{\textbf{id}} & {\textbf{epsrel}} & error & seq. regions & {\textbf{par. regions}} & {\textbf{seq. time}} & {\textbf{par. time}} & {\textbf{speedup}} \\ \hline
%\multirow{Box $s=15$} & 0.001 & 1.3677140579474399e-03 & 2 & 2 & 1.406716 & 1.234737 & 1.14 \\ \cline{2-8}
%  & 3.2e-07 & 6.07465479030012e-08 & 5916 & 15257 & 1790.745862 & 20.341637 & 88.03 \\ \hline
% \multirow{Box $s=22$} & 0.001 & 6.1414786027014201e-04 & 81 & 121 & 45.314449 & 4.5293 & 10.01 \\ \cline{2-8}
%  & 3.2e-07 & 1.05899064406501e-07 & 33308 & 126088 & 11536.390856 & 114.019653 & 101.18 \\ \hline
% \multirow{Corner Peak 3D} & 0.001 & 3.6843437767331e-07 & 7 & 24 & 0.870047 & 4.711789 & 0.18 \\ \cline{2-8}
%  & 3.2e-07 & 8.79007600040893e-09 & 31 & 91 & 2.109112 & 5.017558 & 0.42 \\ \cline{2-8}
%  & 1.024e-10 & 2.70450328798688e-13 & 197 & 1691 & 10.605062 & 7.410759 & 1.43 \\ \hline
% \multirow{CornerPeak 8D} & 0.001 & 1.00574461003866e-06 & 23989 & 25736 & 8552.721608 & 26.463579 & 323.19 \\ \cline{2-8}
%  & 3.2e-07 & 3.06143088657507e-08 & 307592 & 452224 & 435102.763923 & 197.617074 & 2201.75 \\ \hline
% \multirow{$C^0$ 2D} & 0.001 & 2.60485364531604e-05 & 8 & 8 & 0.411517 & 2.184191 & 0.19\\ \cline{2-8}
%  & 3.2e-07 & 1.07664233084392e-09 & 8 & 64 & 0.189059 & 3.377351 & 0.056 \\ \cline{2-8}
%  & 1.024e-10 & 5.77315972805081e-14 & 26 & 512 & 0.472968 & 4.654002 & 0.10 \\ \hline
% \multirow{Gaussian 5D} & 0.001 & 2.03751953711251e-05 & 2396 & 4197408 & 62.469023 & 621.738223 & 0.10 \\ \cline{2-8}
%  & 3.2e-07 & 9.1088385723026e-09 & 166723 & 121221892 & 60264.974689 & 31909.258368 & 1.89 \\ \hline
% \multirow{Corner Peak 6} & 0.001 & 1.2918199069744701e-04 & 112 & 133 & 15.858986 & 6.922758 & 2.29 \\ \cline{2-8}
%  & 3.2e-07 & 1.13556008929372e-07 & 7897 & 11290 & 702.035986 & 10.27877 & 68.29 \\ \cline{2-8}
%  & 1.024e-10 & 8.67184102304464e-12 & 1103754 & 2743278 & 4582929.963441 & 493.321352 & 9289.95 \\ \cline{2-8}
\end{tabular}
\end{table*}

==> integral_test_suite_table.tex <==
\begin{table*}[t]
\caption{Integral Test Suite}
\centering
\begin{tabular}{|c|l|c|c|}
\hline
{\textbf{ID}} & \multicolumn{1}{c|}{{\textbf{Integrand}}} & {\textbf{d}} & Integral \\ \hline
Box s=15 & $(\sum_{i=1}^{d} {x_i}^2)^{s/2}  $ & 8 & 8.87985117541348e3 \\ \hline
Box s=22 & $ (\sum_{i=1}^{d} {x_i}^2)^\frac{22}{2}  $ & 8 & 1.49536928375722e6 \\ \hline
% \multirow{Corner Peak} & $ (1+ \sum_{i=1}^{d} i\cdot x_i)^{-d-1} $ & 3 & $1.08465608465608e-2$ \\ \cline{2-4}
%  & $ (1+ \sum_{i=1}^{d} i\cdot x_i)^{-d-1}$ & 6 & 7.17901606381999e-7 \\ \cline{2-4}
%  & $ (1+ \sum_{i=1}^{d} i\cdot x_i)^{-9} $ & 8 & 2.27519658179178e-10 \\ \hline
% \multirow{Gaussian} & $ e^{-625 \cdot \sum_{i=1}^{d} (x_i-.5)^2}$ & 5 & 1.79132603674879e-6 \\ \cline{2-4}
%  & $ e^{-625 \cdot \sum_{i=1}^{d} (x_i-.5)^2}$ & 8 & 6.38380219000438e-10 \\ \hline
% \multirow{$C^0$} & $-10  \sum_{i=1}^{d} \lvert x_i - .5 \rvert$ & 2 & 3.94627802372637e-2 \\ \cline{2-4}
%  & $-10  \sum_{i=1}^{d} \lvert x_i - .5 \rvert$ & 5 & 3.093636e-4 \\ \cline{2-4}
%  & $-10  \sum_{i=1}^{d} \lvert x_i - .5 \rvert$ & 8 & 2.42521762564189e-6 \\ \hline
% Discontinuous & \begin{tabular}[c]{@{}l@{}}$\begin{cases}\\ 0, & \text{if} z > .9 \\ 0 & \text{if} y > .8 \\ 0 & \text{if} x > .7 \\ 0 & \text{if} w> ,6 \\ 0 & \text{if} v > .5 \\ 0 & \text{if} u > .4\\ e^{10\cdotz + 9\cdoty + 8\cdotx + 7\cdotw + 6\cdotv + 5\cdotu}, \text{otherwise}\\ \end{cases}\\ $\end{tabular} & 6 & 1.54773678850912e8 \\ \hline
\end{tabular}
\end{table*}

==> summary_results_table.tex <==
\begin{table*}[t]
\centering
\caption{Summary Results}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
{\textbf{id}} & {\textbf{epsrel}} & error & seq. regions & {\textbf{par. regions}} & {\textbf{seq. time}} & {\textbf{par. time}} & {\textbf{speedup}} \\ \hline
%\multirow{Box $s=15$} & 0.001 & 1.3677140579474399e-03 & 2 & 2 & 1.406716 & 1.234737 & 1.14 \\ \cline{2-8}
%  & 3.2e-07 & 6.07465479030012e-08 & 5916 & 15257 & 1790.745862 & 20.341637 & 88.03 \\ \hline
% \multirow{Box $s=22$} & 0.001 & 6.1414786027014201e-04 & 81 & 121 & 45.314449 & 4.5293 & 10.01 \\ \cline{2-8}
%  & 3.2e-07 & 1.05899064406501e-07 & 33308 & 126088 & 11536.390856 & 114.019653 & 101.18 \\ \hline
% \multirow{Corner Peak 3D} & 0.001 & 3.6843437767331e-07 & 7 & 24 & 0.870047 & 4.711789 & 0.18 \\ \cline{2-8}
%  & 3.2e-07 & 8.79007600040893e-09 & 31 & 91 & 2.109112 & 5.017558 & 0.42 \\ \cline{2-8}
%  & 1.024e-10 & 2.70450328798688e-13 & 197 & 1691 & 10.605062 & 7.410759 & 1.43 \\ \hline
% \multirow{CornerPeak 8D} & 0.001 & 1.00574461003866e-06 & 23989 & 25736 & 8552.721608 & 26.463579 & 323.19 \\ \cline{2-8}
%  & 3.2e-07 & 3.06143088657507e-08 & 307592 & 452224 & 435102.763923 & 197.617074 & 2201.75 \\ \hline
% \multirow{$C^0$ 2D} & 0.001 & 2.60485364531604e-05 & 8 & 8 & 0.411517 & 2.184191 & 0.19\\ \cline{2-8}
%  & 3.2e-07 & 1.07664233084392e-09 & 8 & 64 & 0.189059 & 3.377351 & 0.056 \\ \cline{2-8}
%  & 1.024e-10 & 5.77315972805081e-14 & 26 & 512 & 0.472968 & 4.654002 & 0.10 \\ \hline
% \multirow{Gaussian 5D} & 0.001 & 2.03751953711251e-05 & 2396 & 4197408 & 62.469023 & 621.738223 & 0.10 \\ \cline{2-8}
%  & 3.2e-07 & 9.1088385723026e-09 & 166723 & 121221892 & 60264.974689 & 31909.258368 & 1.89 \\ \hline
% \multirow{Corner Peak 6} & 0.001 & 1.2918199069744701e-04 & 112 & 133 & 15.858986 & 6.922758 & 2.29 \\ \cline{2-8}
%  & 3.2e-07 & 1.13556008929372e-07 & 7897 & 11290 & 702.035986 & 10.27877 & 68.29 \\ \cline{2-8}
%  & 1.024e-10 & 8.67184102304464e-12 & 1103754 & 2743278 & 4582929.963441 & 493.321352 & 9289.95 \\ \cline{2-8}
\end{tabular}
\end{table*}
